CoCoNets: Continuous Contrastive 3D Scene Representations

This paper explores self-supervised learning of amodal 3D feature representations from RGB and RGB-D posed images and videos, agnostic to object and scene semantic content, and evaluates the resulting scene representations in the downstream tasks of visual correspondence, object tracking, and object detection. The model infers a latent3D representation of the scene in the form of 3D feature points, where each continuous world 3D point is mapped to its corresponding feature vector. The model is trained for contrastive view prediction by rendering 3D feature clouds in queried viewpoints and matching against the 3D feature point cloud predicted from the query view. Notably, the representation can be queried for any 3D location, even if it is not visible from the input view. Our model brings together three powerful ideas of recent exciting research work: 3D feature grids as a neural bottleneck for view prediction, implicit functions for handling resolution limitations of 3D grids, and contrastive learning for unsupervised training of feature representations. We show the resulting 3D visual feature representations effectively scale across objects and scenes, imagine information occluded or missing from the input viewpoints, track objects over time, align semantically related objects in 3D, and improve 3D object detection. We outperform many existing state-of-the-art methods for 3D feature learning and view prediction, which are either limited by 3D grid spatial resolution, do not attempt to build amodal 3D representations, or do not handle combinatorial scene variability due to their non-convolutional bottlenecks.

==> 2_intro_final.tex <==
%\vspace{-1em}
\section{Introduction} \label{sec:intro}

For visual perception models to generalize beyond the domain they are trained on, it is important for the models to learn or improve their feature representations self-supervised. % feature learning has emerged as an important direction for learning visual feature representations  within 
The current approach involves training on a pretext task which does not require human annotations, such as view/frame/context  prediction, with the hope of learning representations useful for downstream semantic tasks, such as object detection, tracking, manipulation and navigation  
\cite{Eslami1204,commonsense,adam3d,lee2017unsupervised,DBLP:journals/corr/DoerschGE15,pathakCVPR16context,DBLP:journals/corr/ZhangIE16,DBLP:journals/corr/abs-1806-09594,oord2018representation,sermanet2018timecontrastive}.
Many of these downstream tasks require reasoning about free space, scene and object occupancy, correspondence of objects and parts across time and space,  understanding camera motion, and invariance to cross-object occlusions \cite{weng2020ab3dmot,nagabandi2019deep}. 
%1. learn features by moving
Understanding the three-dimensional structure of  objects and  scenes  may be a key for success in these tasks, as well as generalization of perception across camera viewpoint and scene variations.  

Exciting recent works have explored learning representations of objects and scenes from multiview imagery and capture the three-dimensional scene structure implicitly or explicitly with  3D binary or feature grids \cite{DBLP:journals/corr/TulsianiZEM17,TulGupFouEfrMal17,sitzmann2018deepvoxels}, 3D point feature clouds \cite{Wiles_2020_CVPR},  implicit functions that map continuous world coordinates to  3D point occupancy  \cite{chibane2020implicit,genova2020local,sitzmann2020scene, mescheder2019occupancy, park2019deepsdf, chen2019learning}, as well as 1D or 2D feature maps \cite{Eslami1204}. 
%Many of the methods above are trained without explicit 3D supervision through differentiable rendering routines %that incorporate a variable amount of domain knowledge,
%, object-centric feature maps \cite{}, and is trained 
%by predicting image views \cite{Eslami1204,sitzmann2020scene}. 
These methods typically evaluate  the accuracy of the inferred 3D scene occupancy  \cite{chibane2020implicit,novotny2020canonical,DBLP:journals/corr/TulsianiZEM17, mescheder2019occupancy, park2019deepsdf, chen2019learning} and the fidelity of   image views rendered from the 3D representation \cite{le2020novel,mildenhall2020nerf,Eslami1204,Wiles_2020_CVPR,sitzmann2020scene}, as opposed to the suitability of representations for downstream semantic tasks. 
Methods that indeed focus on rendering photo-realistic images often give up on cross-scene generalization \cite{mildenhall2020nerf,riegler2020free}, or focus on single-object scenes \cite{sitzmann2020scene}. 
%Methods that do target feature representation learning, if they lack explicit 3D inductive biases in their architecture, have difficulty generalizing to novel scenes. 
Methods that instead focus on learning semantically relevant scene representations are expected to generalize across scenes, and handle multi-object scenes. 
In the 2D image space, contrastive predictive coding  has shown to generate state-of-the-art visual features for correspondence and recognition \cite{oord2018representation,han2019video}, but does not encode  3D scene structure.  
In 3D voxel feature learning methods  \cite{adam3d,harley2020tracking}, convolutional latent 3D feature grids encode the 3D structure and a view contrastive objective learns semantically useful 3D representations, but  the  grid resolution limits the discriminability of the features learnt. % Voxel grids and the convolutional nature of those networks permit such generalization \cite{commonsense,adam3d}, however the grid resolution limits the discriminability of the features learnt. 
Recent exciting works combine 3D voxel grids and implicit functions and learn to  predict 3D scene and object 3D occupancy from a single view with unlimited spatial resolution \cite{peng2020convolutional,popov2020corenet}.  
The model proposed in this work brings together these two powerful ideas: 3D  feature grids 
as a 3D-informed neural bottleneck for contrastive view prediction \cite{adam3d}, and implicit functions for handling the resolution limitations of 3D  grids \cite{peng2020convolutional}. % and contrastive predictive coding \cite{oord2018representation} for unsupervised training of 3D feature representations by predicting views.

%Our question then in this paper is: could we combine 3D voxel implicit representations and contrastive view prediction to learn 3D feature representations of infinite spatial resolution, useful for object tracking and correspondence? %, by simply moving around and collecting posed RGB-D images?

% evaluation on rendering/occupancy rather than feature learning

% lack of generalization across viewpoints/scene if 1) fully connected or not in 3D.

%

%captured either as explicit 3D grids, 3D feature clouds or implicit functions.  
%Amodal complete 3D representations are much easier to track and correspond in comparison to single  view image features, prone to drifting due to occlusions and dis-occlusions of object content. 
%Humans are capable of such 3D amodal completion from single view, yet, machine learning models have just started to address such ability by inferring from images models that can predict  views of a scene and objects occluded in the input image.


%Many classic explicit 3D scene representations, such as voxel occupancy grids [5–10], point clouds [11–14], or meshes [15] have been integrated with end-to-end deep learning models  and have led to significant progress in 3D scene understanding. 

%Many recent works learn 3D object shape with functional form, in terms of a neural network that given an XYZ coordinate predicts occupancy and a feature vector for the corresponding point, to handle resolution limitations of voxelization.

%The methods above have been mostly used for rendering compelling RGB images of single objects or simple scenes or high accurate 3D occupancies, and mostly focus on such image generation ability as opposed to the utility of the emergent feature representations for recognition and visual correspondence. Also, most of the methods work on objects in isolation and have difficulty generalizing across realistic scenes with multiple objects and varying object number and appearance.

We propose Continuous Contrastive 3D Networks (\model), a model that learns to map RGB-D images to infinite-resolution 3D scene feature representations by contrastively predicting views, in an object and scene agnostic way. 
% \ishita{Moreover, we will later show how \model{} can be extended to use just the RGB images for the task of view regression and point alignment.}
% that are useful for downstream tasks of recognition and detection.
% They lift RGB-D (2.5D) views to \todo{feature function grids and renders 3D point features to generate the corresponding 2D feature maps by concurrently training a 2D CNN in an end-to-end differentiable manner. }
Our model is trained to predict views of static scenes given 2.5D (color and depth; RGB-D) video streams as input, and is evaluated on its ability to detect and recognize objects in 3D. 
Our model maps the 2.5D input streams into 3D feature grids of the depicted scene. %At every frame, the architecture accounts for the motion of the camera, so that the internal 3D representation remains stable under egomotion. 
Given a target view and its viewpoint, 
the model first warps its inferred 3D feature map from the input view to a target view, then queries point features using their continuous coordinates,  and pulls these features closer to the point features extracted from the target view at the same 3D locations (Figure \ref{fig:model}). We use a contrastive loss to measure the matching error, and backpropagate gradients end-to-end to our differentiable modular architecture. At test time, our model forms plausible 3D completions of the scene given a \textit{single RGB-D image} as input: it learns to fill in information behind occlusions, and infer the 3D extents of objects. Moreover, we show how \model{} can also be extended to use just the RGB images for the task of view regression and point alignment. %\usepackage}

We demonstrate the advantages of combining 3D neural bottleneck, implicit functions and contrastive learning for 3D representation learning 
by comparing our model against state-of-the-art self-supervised models, such as i) contrastive learning for pointclouds \cite{xie2020pointcontrast}, which shares a similar loss but not the amodal predictive ability of our model, ii) contrastive neural mapping \cite{harley2020tracking}, which can amodally inpaint a 3D discrete feature grid but suffers from limited spatial grid resolution, and iii) dense  ObjectNets \cite{pmlr-v87-florence18a}, which self-learns  2D (instead of 3D) feature representations with a similar triangulation-driven supervision.  
Our experimental results can be summarized as follows:
\textbf{(1)} 3D object tracking and re-identification (Figure \ref{fig:tracking_quali}): We show that   scene representations learnt by \model{} can detect objects in 3D across large frame gaps better than the baselines  \cite{xie2020pointcontrast,harley2020tracking,pmlr-v87-florence18a}.
%outperform the SOTA method in tracking 3D objects. 
\textbf{(2)} Supervised 3D object detection: Using the learnt 3D point features as initialization  boosts the performance of the state-of-the-art Deep Hough Voting detector of \cite{qi2019deep}. \textbf{(3)} 3D cross-view and  cross-scene object 3D alignment: We show that the learnt 3D feature representations can infer 6DoF alignment between the same object in different viewpoints, and across different objects of the same category, better than  \cite{xie2020pointcontrast,harley2020tracking,pmlr-v87-florence18a}. 
 %, and show superior performance %With these comparisons we demonstrate the advantages of combining 3D neural bottleneck, implicit functions and contrastive learning for 3D representation learning. 
We further show that our model can predict image views (with or without depth as input) and 3D occupancies that outperform or are on par with the state-of-the-art view and occupancy prediction models \cite{popov2020corenet,commonsense,Eslami1204}.


In summary, the main contribution of this paper is a model that learns  infinite-resolution 3D scene representations from  RGB-D posed images,  useful for tracking and corresponding objects in 3D, pre-training  3D object detectors, and predicting views and 3D occupancies. We set a new state-of-the-art  in self-supervision of 3D feature representations. %Our data and code will be made publicly available.%Our model further predicts RGB image views and 3D occupancies and can generalize to truly novel scenes. %To the best of our knowledge, our work is the first to learn amodal 3D representations are the first to extract high-quality  3D features.
%general scenes and objects that would permit object matching and object tracking or across instance feature matching, and thus by useful for downstream recognition tasks as opposed to solely single object 3D occupancy prediction? 



%Importantly, methods seeking explicit 3D object reconstruction in terms of .. may not be necess

% view prediction has shown to be a scalable self-supervised objective for learning visual representations where the 3D structure of the world is captured implicitly, by a functional form, or using 
 
 
 %supervised from egomotion and depth of world scenes that are useful for downstream visual recognition tasks like object detection and tracking. The representations which are found to generalize in this domain are the ones that use use 3D latent maps as their bottleneck representation. The generalization of these methods can be attributed to their explicit architectural biases which ensures camera viewpoint in-variance and translational equivariance.



%an important constraint or inductive bias to impose during such self-supervised training. 


%Predicting views has shown to be 
%Recent approaches have shown  view prediction to be 
%a scalable objective for learning visual feature representations supervised from egomotion and depth of world scenes that are useful for downstream visual recognition tasks like object detection and tracking.


%A recent streams of work focus on extracting 3D 


%A major driver behind recent work on generative models has been the promise of unsupervised discovery of powerful neural scene representations, enabling downstream tasks ranging from robotic manipulation and few-shot 3D reconstruction to navigation. A key aspect of solving these tasks is understanding the three-dimensional structure of an environment. However, prior work on neural scene representations either does not or only weakly enforces 3D structure [1–4]. Multi-view geometry and projection operations are performed by a black-box neural renderer, which is expected to learn these operations from data. As a result, such approaches fail to discover 3D structure under limited training data (see Sec. 4), lack guarantees on multi-view consistency of the rendered images, and learned representations are generally not interpretable. Furthermore, these approaches lack an intuitive interface to multi-view and projective geometry important in computer graphics, and cannot easily generalize to camera intrinsic matrices and transformations that were completely unseen at training time.
%In geometric deep learning, many classic 3D scene representations, such as voxel grids [5–10], point clouds [11–14], or meshes [15] have been integrated with end-to-end deep learning models and have led to significant progress in 3D scene understanding. However, these scene representations are discrete, limiting achievable spatial resolution, only sparsely sampling the underlying smooth surfaces of a scene, and often require explicit 3D supervision.

%We propose a method for amodal 3D scene feature learning supervised by predicting views



